Graphical Methods in Device-Independent Quantum Cryptography

We introduce a framework for graphical security proofs in device-independent quantum cryptography using the methods of categorical quantum mechanics. We are optimistic that this approach will make some of the highly complex proofs in quantum cryptography more accessible, facilitate the discovery of new proofs, and enable automated proof verification. As an example of our framework, we reprove a previous result from device-independent quantum cryptography: any linear randomness expansion protocol can be converted into an unbounded randomness expansion protocol. We give a graphical proof of this result, and implement part of it in the Globular proof assistant.

==> tikzstyles.tex <==
% Created using Coecke & Kissinger's style files + help files from the
% internet.

% The following TiKz styles are declared in this file:

% NODE STYLES:
% "spider" (spider)
% "qspider" (quantum spider)
% "qprocess" (quantum process)
% "qprocessxflip" (quantum process)
% "qprocessyflip" (quantum process)
% "qprocessxyflip" (quantum process)
% "cprocess" (classical process)
% "cprocessxflip" (classical process)
% "cprocessyflip" (classical process)
% "cprocessxyflip" (classical process)
% "qstate" (quantum state)
% "qstatexflip" (quantum state, conjugated)
% "qeffect" (quantum effect)
% "qeffectxflip" (quantum effect, conjugated)
% "cstate" (classical state)
% "cstatexflip" (classical state, conjugated)
% "ceffect" (classical effect)
% "ceffectxflip" (classical effect, conjugated)
% "terminal" (terminal process)
% "initial" (initial process)
% "uniform" (classical uniform state)
% "quniform" (bell state)
% "scalar" (scalar)

% EDGE STYLES:
% "cedge" (classical edge)
% "qedge" (quantum edge)

% Note that we can specify anchors to a qprocess as cardinal
% directions (e.g., def.south) or as numbers (e.g., def.90).  If we
% want an edge to curve, we can do so by adding parameters like
% "in=-90", "out=90" to the arguments.

% Here is some example code:

% -- BEGIN EXAMPLE
%\begin{tikzpicture}
%\node (firstpoint) at (0,2) {};
%\node[style=qprocess] (abc) at (0,0) {abc};
%\node[style=cprocessxyflip] (def) at (1,1) {def};
%\node (lastpoint) at (1,-1) {};
%\node[style=spider] (spider1) at (1,2) {};
%\draw[style=qedge] (spider1) to (def);
%\draw[style=qedge] (abc) to (def.south);
%\draw[style=qedge] (lastpoint) to (abc);
%\end{tikzpicture}
% -- END EXAMPLE

\makeatletter
\usetikzlibrary{circuits.ee.IEC}

\def\declaretrapezoid#1#2#3#4#5{
\pgfdeclareshape{#1}{
\inheritsavedanchors[from=rectangle]
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{east}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{south east}
\inheritanchor[from=rectangle]{north west}
\inheritanchor[from=rectangle]{north east}
\inheritanchor[from=rectangle]{south west}

\backgroundpath{
  \pgfextractx{\pgf@xa}{\southwest}
  \pgfextracty{\pgf@ya}{\southwest}
  \pgfextractx{\pgf@xb}{\northeast}
  \pgfextracty{\pgf@yb}{\northeast}

  \pgfpathmoveto{\pgfpoint{\pgf@xa-#2*(\pgf@yb-\pgf@ya)}{\pgf@ya}}
  \pgfpathlineto{\pgfpoint{\pgf@xa-#3*(\pgf@yb-\pgf@ya)}{\pgf@yb}}
  \pgfpathlineto{\pgfpoint{\pgf@xb+#4*(\pgf@yb-\pgf@ya)}{\pgf@yb}}
  \pgfpathlineto{\pgfpoint{\pgf@xb+#5*(\pgf@yb-\pgf@ya)}{\pgf@ya}}
  \pgfpathlineto{\pgfpoint{\pgf@xa-#2*(\pgf@yb-\pgf@ya)}{\pgf@ya}}
  }
  }
}

\pgfdeclareshape{clipped triangle}{
\inheritsavedanchors[from=rectangle]
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{east}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{south east}
\inheritanchor[from=rectangle]{north west}
\inheritanchor[from=rectangle]{north east}
\inheritanchor[from=rectangle]{south west}

\backgroundpath{
  \pgfextractx{\pgf@xa}{\southwest}
  \pgfextracty{\pgf@ya}{\southwest}
  \pgfextractx{\pgf@xb}{\northeast}
  \pgfextracty{\pgf@yb}{\northeast}

  \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
  \pgfpathlineto{\pgfpoint{\pgf@xb+0.5*(\pgf@xb - \pgf@xa}{\pgf@ya}}
  \pgfpathlineto{\pgfpoint{0.6*\pgf@xa + 0.4*\pgf@xb)}{\pgf@yb+0.5*(\pgf@yb-\pgf@ya)}}
  \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
  \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
  }
}

\pgfdeclareshape{clipped triangle xflip}{
\inheritsavedanchors[from=rectangle]
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{east}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{south east}
\inheritanchor[from=rectangle]{north west}
\inheritanchor[from=rectangle]{north east}
\inheritanchor[from=rectangle]{south west}

\backgroundpath{
  \pgfextractx{\pgf@xa}{\southwest}
  \pgfextracty{\pgf@ya}{\southwest}
  \pgfextractx{\pgf@xb}{\northeast}
  \pgfextracty{\pgf@yb}{\northeast}

  \pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@ya}}
  \pgfpathlineto{\pgfpoint{\pgf@xa+0.5*(\pgf@xa - \pgf@xb}{\pgf@ya}}
  \pgfpathlineto{\pgfpoint{0.6*\pgf@xb + 0.4*\pgf@xa)}{\pgf@yb+0.5*(\pgf@yb-\pgf@ya)}}
  \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
  }
}

\pgfdeclareshape{clipped triangle xyflip}{
\inheritsavedanchors[from=rectangle]
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{east}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{south east}
\inheritanchor[from=rectangle]{north west}
\inheritanchor[from=rectangle]{north east}
\inheritanchor[from=rectangle]{south west}

\backgroundpath{
  \pgfextractx{\pgf@xa}{\southwest}
  \pgfextracty{\pgf@ya}{\southwest}
  \pgfextractx{\pgf@xb}{\northeast}
  \pgfextracty{\pgf@yb}{\northeast}

  \pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  \pgfpathlineto{\pgfpoint{\pgf@xa+0.5*(\pgf@xa - \pgf@xb}{\pgf@yb}}
  \pgfpathlineto{\pgfpoint{0.6*\pgf@xb + 0.4*\pgf@xa)}{\pgf@ya+0.5*(\pgf@ya-\pgf@yb)}}
  \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
  \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  }
}

\pgfdeclareshape{clipped triangle yflip}{
\inheritsavedanchors[from=rectangle]
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{east}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{south east}
\inheritanchor[from=rectangle]{north west}
\inheritanchor[from=rectangle]{north east}
\inheritanchor[from=rectangle]{south west}

\backgroundpath{
  \pgfextractx{\pgf@xa}{\southwest}
  \pgfextracty{\pgf@ya}{\southwest}
  \pgfextractx{\pgf@xb}{\northeast}
  \pgfextracty{\pgf@yb}{\northeast}

  \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}
  \pgfpathlineto{\pgfpoint{\pgf@xb+0.5*(\pgf@xb - \pgf@xa}{\pgf@yb}}
  \pgfpathlineto{\pgfpoint{0.6*\pgf@xa + 0.4*\pgf@xb)}{\pgf@ya+0.5*(\pgf@ya-\pgf@yb)}}
  \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
  \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
  }
}

\declaretrapezoid{right-in trapezoid}{0}{0}{0.5}{0}
\declaretrapezoid{right-out trapezoid}{0}{0}{0}{0.5}
\declaretrapezoid{left-in trapezoid}{0}{0.5}{0}{0}
\declaretrapezoid{left-out trapezoid}{0.5}{0}{0}{0}

\tikzstyle{terminal}=[circuit ee IEC, ground, thick, rotate=90]
\tikzstyle{initial}=[circuit ee IEC, ground, thick, rotate=-90]

\tikzstyle{cedge}=[swap]
\tikzstyle{qedge}=[swap,very thick]

\tikzstyle{qprocess}=[draw,very thick,shape=right-in trapezoid]
\tikzstyle{qprocessxflip}=[draw,very thick,shape=left-out trapezoid]
\tikzstyle{qprocessyflip}=[draw,very thick,shape=right-out trapezoid]
\tikzstyle{qprocessxyflip}=[draw,very thick,shape=left-out trapezoid]

\tikzstyle{qeffect}=[draw,very thick,shape=clipped triangle]
\tikzstyle{qeffectxflip}=[draw, very thick,shape=clipped triangle xflip]
\tikzstyle{qstatexflip}=[draw, very thick,shape=clipped triangle xyflip]
\tikzstyle{qstate}=[draw, very thick,shape=clipped triangle yflip]

\tikzstyle{ceffect}=[draw,shape=clipped triangle]
\tikzstyle{ceffectxflip}=[draw, shape=clipped triangle xflip]
\tikzstyle{cstatexflip}=[draw, shape=clipped triangle xyflip]
\tikzstyle{cstate}=[draw, shape=clipped triangle yflip]

\tikzstyle{cprocess}=[draw,shape=right-in trapezoid]
\tikzstyle{cprocessxflip}=[draw,shape=left-in trapezoid]
\tikzstyle{cprocessyflip}=[draw,shape=right-out trapezoid]
\tikzstyle{cprocessxyflip}=[draw,shape=left-out trapezoid]

\tikzstyle{spider}=[draw,shape=circle]
\tikzstyle{qspider}=[draw,very thick,shape=circle]

\tikzstyle{uniform}=[draw,shape=circle,fill=gray]
\tikzstyle{quniform}=[draw,very thick,shape=circle,fill=gray]

\tikzstyle{scalar}=[draw,shape=diamond]

\tikzstyle{scp}=[draw,very thick,shape=rectangle]

\tikzstyle{process}=[draw,shape=rectangle]

